Survey on UAV Cellular Communications: Practical Aspects, Standardization Advancements, Regulation, and Security Challenges

The rapid growth of consumer Unmanned Aerial Vehicles (UAVs) is creating promising new business opportunities for cellular operators. On the one hand, UAVs can be connected to cellular networks as new types of user equipment, therefore generating significant revenues for the operators that can guarantee their stringent service requirements. On the other hand, UAVs offer the unprecedented opportunity to realize UAV-mounted flying base stations that can dynamically reposition themselves to boost coverage, spectral efficiency, and user quality of experience. Indeed, the standardization bodies are currently exploring possibilities for serving commercial UAVs with cellular networks. Industries are beginning to trial early prototypes of flying base stations or user equipments, while academia is in full swing researching mathematical and algorithmic solutions to address interesting new problems arising from flying nodes in cellular networks. In this article, we provide a comprehensive survey of all of these developments promoting smooth integration of UAVs into cellular networks. Specifically, we survey (i) the types of consumer UAVs currently available off-the-shelf, (ii) the interference issues and potential solutions addressed by standardization bodies for serving aerial users with the existing terrestrial base stations, (iii) the challenges and opportunities for assisting cellular communications with UAV-based flying relays and base stations, (iv) the ongoing prototyping and test bed activities, (v) the new regulations being developed to manage the commercial use of UAVs, and (vi) the cyber-physical security of UAV-assisted cellular communications.

==> ChannelModel.tex <==
\graphicspath{{Figures/}}
\section{Channel Model} \label{s:channelmodel}

%Considering the exponential use of UAVs and drones in cellular communication, developing a new channel model compatible with UAV characteristics is necessary.
%In this Section, we categorized the channel model specifications into three main categories, including Air to Ground (A2G), Ground to Air (G2A), and Air to Air (A2A). In each category, field experiments as well as analytical and simulation works are addressed and described in details.

{\bf [LORENZO] IN THIS SECTION WE NEED TO REMOVE ANY REFERENCE TO STUDIES AND TRIALS WHO HAVE BEEN TAKEN AS A REFERENCE BY 3GPP AND CITED EARLIER IN THE STANDARDIZATION SECTION. I WOULDN'T REMOVE THIS PART AS DISCUSSED BEFORE, BUT MAYBE JUST CUT A BIT HERE AND THERE.}

Considering the exponential use of UAVs and drones in cellular communication, developing a new channel model able to capture all the new UAV specific characteristics is necessary. On top of the model that has been officially approved by 3GPP for conducting UAV studies, and already described in Section \ref{subs:channelmodelling}, a variety of field experiments as well as analytical and simulation studies have been conducted by the research community. 
In this Section, we categorized the channel model specifications into three main categories, including Air to Ground (A2G), Ground to Air (G2A), and Air to Air (A2A). 

%%%%%%%

\subsection{Air-to-Ground}

\begin{table*}[]
	\centering
	\caption{ITU environmental parameters}
	\label{tbl:itu_param_env}
	\begin{tabular}{|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{Parameters} & \multirow{2}{*}{Definition} & \multicolumn{4}{c|}{Values}         \\ \cline{3-6} 
		&                             & Suburban & Urban & Dense & Highrise \\ \hline
		$\alpha$& Ratio of built-up land area to the total land area   &  0.1&  0.3   &0.5   & 0.5  \\ \hline
		$\beta$&      The mean number of buildings per unit area  &     750     & 500      & 300      &  300        \\ \hline
		$\gamma$&  A scale parameter that describes the buildings heights distribution &     8     &   15    & 20      &  50        \\ \hline
	\end{tabular}
\end{table*}

The air to ground channel is studied by researchers through field experiments and simulations.
In this section we first review the works involving experiments to identify the channel specifications.

Qualcomm conducted field experiments \cite{qualcommuavtr} in California, where a custom-designed  quadrotor drone is used at the maximum height of 120m (height of 30m, 60m, 90m, and 120m) in three different LTE bands (PCS, AWS, and 700MHz). The results shows that the number of detected cells increases with altitude. The longer propagation distance of signals  in the free space is the reason of such observation. Moreover, the measured path loss at different altitudes are compared with the free space path loss. The results indicate that the free space model (with path loss exponent 2) is an acceptable model for air to ground communications. 
%
Additionally, NASA has a project titled "UAS integration in the National airspace System", one of its goal is to study the characteristic of the channel for air to ground communication. Part of the experiment results of NASA projects are reported in \cite{7357682} and \cite{sun2015dual}. In these experiments, a S-3B Viking aircraft at the hight of 560m is utilized in 970Mhz (L-band), and 5060MHz (C-band). An omnidirectional blade monopole antenna is mounted on the bottom of aircraft.
The path loss between a ground station and the aircraft is measured, where the link distance between them varies from 1.7Km to 19Km. It was shown that the log-distance path loss model is more fitted with the experimental results, as follows:

\begin{equation}
P_{LoS}(d)=A_0+10n\log(d/d_{min})+X
\label{eq:NASApathloss}
\end{equation} 
where $A_0$ denotes the path loss at the minimum distance $d_{min}$ of 1.7 km, $n$ denotes the path loss exponent, and $X$ is a zero mean Gaussian random variable. The value of $A_0$ is 113.9 dB, and 102.3 dB for the C-band and L-band receivers, respectively. In these experiments, a path loss exponent ($n$) of 1.6 in L-band and 1.9 in C-band are founded. 
%
Amorim et al. \cite{7936620} conducted field measurement using a commercial UAV in 800MHz frequency in Denmark, to model the path loss exponent and shadowing for UAV communication at the height of up to 120m. The path loss exponent is then driven based on the received signal power from detected cells and their distances. The experiments show that the path loss exponent reduces considerably as the UAV moves up, and becomes closer to the free space propagation at higher height. Moreover, results show that the shadowing variation also reduces by increasing the UAV height. The shadowing variation decrease from 6.4(dB) to 3.2(dB) for the height of 15m and 120m respectively. The main contribution of this work is proposing a height dependent model for path loss and shadowing in UAV communications. Some of the measured path loss exponent through different studies are summarized in Table \ref{tbl:A2Gpathlossexp}.
%
Authors in \cite{8048502} also have done extensive filed measurements in Australia in order to evaluate the channel model for ground to air communications. They tried to model the channel based on the existed terrestrial channel model and considering an excess path loss exponent on top of it for the ground to air communications. Interestingly, they found that the path loss mainly depends on the elevation angle between the UAV and the base stations. According to their measurements, the excess path loss exponent reduces by increasing the elevation angle, as the UAV becomes closer to the base station. However, at some point the effect of down-tilted base station antenna dominated and the path loss increases. The experiments have done in 850MHz frequency using LTE technology, and the excess aerial path loss are modeled based on elevation angle, and some experimental fitting parameters.

%%%%%%simulation
As mentioned before, simulation model is another way to characterize the channel specifications. The feasibility of modeling multiple UAVs and ground stations is one of the main advantages of the simulation. In the following, the recent studies involving simulations and analytical models are reviewed.

For aerial UEs communications with different types of base stations, such as rural macro BS, urban macro BS, and urban micro BS, a LoS probability function is provided by 3GPP in \cite{3GPP36777}, where mainly depends on the UAV height and its 2D distance from the BS. The antenna heights of 35m for rural macro BS, 25m for urban macro BS, and 10m for urban micro BS are assumed in this work. 
Figure \ref{fig:umiplos} illustrate the impact of UAV height and 2D distance on LoS probability for urban micro BSs. According to this figure, higher 2D distance reduces the probability of having a LoS connection between the UAV and the urban micro BS. Additionally, at higher UAV height, there is a larger probability of having LoS.
%In this model, there is a 100\% LoS connection when aerial UE is flying above 100m height. 
A path loss model and a log normal shadow fading model are introduced in this work for aerial UEs as well. According to \cite{3GPP36777}, the height of UAV, frequency, and the distance have the major impact in modeling the path loss and shadowing. The impact of frequency and distance on path loss is shown in Figure \ref{fig:plurbanmicro}. As illustrated in this figure, the path loss increases by increasing the distance between the UAV and the BS. Also it observed that higher frequency generates slightly higher path loss value.
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{umiplos-dis.pdf}
	\caption{LoS probability between an urban micro BS and UAV at different height}
	\label{fig:umiplos}
\end{figure}
%
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{plurbanmicro.pdf}
	\caption{Path loss for a communication between an urban micro BS and UAV at 50m height}
	\label{fig:plurbanmicro}
\end{figure}

The path loss for air to ground communications is studied in \cite{7037248} for low altitude platform.
At first, the International Telecommunication Union (ITU) statistical urban parameters \cite{ITU} are used to simulate the environment. ITU has suggested a model for describing different urban environments (suburban, urban, dense and highrise urban) based on three parameters. The ITU parameters and their values are summarized in Table \ref{tbl:itu_param_env}. Utilizing ITU parameters, a virtual Manhattan-model city of size 1000$\times$1000 is simulated using MATLAB.
Moreover, Wireless InSite software is used to model the ray tracing including three types of ray (direct, reflected and diffracted).
The simulation is conducted for four different environments and three different frequencies namely, 700MHz, 2000 MHz and 5800MHz. It is assumed that the UAV is located  at a height between 200m and 3000m, and ground users are distributed uniformly in the area. The excessive path loss over the free space path loss is calculated. The results show that the receivers mostly enjoy a LoS connection (direct ray), while only 3\% percentage of the communications suffer from diffracted propagations and high path loss. The value of excess path loss for direct propagation group is reported in Table \ref{tbl:A2Gpathlossexp}.
Based on the simulation results, a model to find the probability of a certain propagation groups is defined, which depends on altitude, elevation angle (See Figure \ref{fig:params}) and ITU urban parameters.
\begin{figure}
	\centering
	\includegraphics[width=0.9\linewidth]{params}
	\caption{Definition of parameters in UAV communications}
	\label{fig:params}
\end{figure}
Unlike \cite{7037248} that models the urban area using the Manhattan grid, typical European cities with irregular street size and orientation are modeled in \cite{4151547}. In this work, the probability of a having a LoS connection is modeled as Equation (\ref{eq:pathlossirreg}),
\begin{equation}
P_{LoS}(\theta)= 1- \frac{H-h_r}{w_s}\sin(\alpha)\cot(\theta)
\label{eq:pathlossirreg}
\end{equation} 
where $H$ denoted the average building height, $w_s$ is the average street length, and $\theta$ shows the elevation angle. Moreover, $\alpha$ is defined as the street angle.
The model is evaluated through ray tracing simulation software where the airborn node can be located at the height of 100m, 200m, 500m, 1000m and 2000m. The simulation results shows that the derived model is compatible with the LoS probabilities extracted from local geographical data. Higher elevation angle increases the probability of LoS in this model.

Experimental and simulation works are summarized in Table \ref{tbl:channel_exp} and \ref{tbl:channel_simul}, respectively.

%\paragraph{3gpp to be work on it}

\begin{table}[]
	\centering
	\caption{Summary of A2G path loss exponent (PLE)}
	\label{tbl:A2Gpathlossexp}
	\begin{tabular}{|m{0.7cm}|m{1.6cm}|m{4.5cm}|}
		\hline
		\textbf{Ref.} & \textbf{PLE} & \textbf{Description}\\ \hline
		\cite{qualcommuavtr}&2& maximum height= 120m, PCS, AWS, and 700MHz \\ \hline
		\cite{7470935}&2.32& height=20m, ZigBee 802.145.4 \\ \hline
		\cite{7357682}& 1.6 &  height=560m, speed = 71m/s,  970Mhz (L-band) \\ \hline
		\cite{7357682}&  1.9 &  height=560m, speed = 71m/s, 5060MHz (C-band) \\ \hline
		\cite{7037248}& 0 (suburban)*\newline 0.6 (urban) \newline 1 (Dense) \newline 1.5 (Highrise)&height = below 3000m, quasi-stationary, 700MHz\newline * (values show excessive path loss)\\ \hline
		\cite{7936620}&2.9&height=15m, speed = 15km/h,  800Mhz\\ \hline
		\cite{7936620}&2.5&height=30m, speed = 15km/h,  800Mhz\\ \hline
		\cite{7936620}&2.1&height=60m, speed = 15km/h,  800Mhz\\ \hline
		\cite{7936620}&2&height=120m, speed = 15km/h,  800Mhz\\ \hline
	\end{tabular}
\end{table}


%\paragraph{Old Air-to-Ground}

%ITU urban parameters are also used in \cite{sharmastudy} in urban environment simulator to analyze the channel model for air to ground transmission. It is assumed that the UAV can fly at the height of  100m to 2000m, equipped with a isotropic antenna with a power of 18dBm , and 2.44GHz frequency. The simulation results present the high dependency of path loss and shadowing on elevation angle and the UAV height. 
%The probability of LoS for low altitude airborne stations (up to 10000m) is addressed in \cite{6863654}, according to the following equation:
%\begin{equation}
%P_{LoS}(\theta)=\frac{1}{1+ a.e^{-b(\theta-a)}}
%\label{eq:pathloss6863654}
%\end{equation} 
%where $\theta$ is the elevation angle and $a$ and $b$ are environmental parameters.
%
% Moreover, filed measurements in \cite{7470934} prove that a new channel model for integrating UAVs in cellular network is required, specially because of interference signals and change of path loss exponent. Two different scenarios are studied in this work, where in the first scenario, the UAV acts as a UE and communicates with a ground base station having a down-tilt antenna. In the second scenario, the UAV is employed as a base station, hovering at the height of 150m.
%%
%
%%%%%%%%%
%\cite{ikram2017tier}
%Considering a more precise air-to-ground channel (AtG)
%model that incorporates temperature, wind, foliage, nearsea
%environments, urban environments is crucial for a
%more precise performance analysis. This is a potential
%future direction to work on.
%
%%%%%%%%
%Impact of rain, cloud and gaseous absorption for air to ground communication in high altitude using simulation are also analyzed in \cite{6685719}. The simulation is conducted for the frequencies above 10GHz, where gaseous absorption, cloud and rain have a major effect on transmissions. The simulation results presented that the attenuation of these parameters goes higher in the higher frequencies. Moreover,. it is shown that among these parameters, rain attenuation has the major impact on transmissions. 
% 
%%other tryies to characterize the channel model
%Although many studies are trying to characterize the path loss exponent for air to ground communication, \cite{7842372} focuses on the large scale fading, small scale fading, and multipath propagation. In this work,
%Intensive experiments with a UAV at the height of 4m to 16m, and a facing down antenna are conducted in Florida university. Ultra wideband frequencies of 3.1GHz to 5.3GHz are selected for these experiments. Results show that when UAV moves additional path loss and shadowing variances are introduced. Moreover, more fading is observed when UAV is located at higher height. The experiments cover open area and sub urban area as well, and the results show more variance in small scale channel characteristics in sub urban area rather than open area. The existence of more reflection and scattering in urban area could be one reason to this phenomena.
%
%Path loss model for very high altitude platform, in the range of 17Km to 22Km, is investigated in \cite{4483593} for different urban area by simulation. The following equation expressed the proposed model for the probability of LoS between the airborne station and ground users:
%\begin{equation}
%P_{LoS}(\theta)=a-{\frac{a-b}{1+(\frac{\theta-c}{d})^{e}}}
%\label{eq:pathloss4483593}
%\end{equation} 
%where $\theta$ is the elevation angle, and $a,b,c,$ and $d$ are environmental parameters. The aircraft transmits over the frequencies of 2GHz, 3GHz, and 5.5GHz, with a patch antenna. Ground receivers is assumed to have a spiral broadband antennas.
%A shadowing model for high altitude platforms in built-up areas is modeled in \cite{loke2015internet}. 
%%\cite{liu2017performance}
%



\subsection{Ground-to-Air}
In addition to the air to ground links, ground to air links need to be studied, as researchers show that they may have different specifications \cite{7470935}. 
In this section we review the recent works on ground to air links.

\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{rxfacing}
	\caption{Four receivers mounted on the UAV with different directions \cite{5700251}}
	\label{fig:rxfacing}
\end{figure}

Fields experiments are used in several studies to realize the G2A channel specifications. For example, the measured RSSI between a ground station and a hexacopter at the height of 20m, shows  a path loss exponent of 2.51 for ground to air communications \cite{7470935}. The measured path loss exponent for other types of links are summarized in Table \ref{tbl:estimaedpathlossallLinks}.
Results reveal that the path loss exponent for A2G is slightly better than G2A links.
%%%%
More experiments using fix-wing fuselag at the altitude of 75m are conducted in \cite{5700251}. In these experiments, four different receiver antennas facing at various directions are mounted on the UAV to receive data from a fixed ground station. Two of the receivers faced downward, one of them faced skyward and the last one faced the bow to provide diversity in antenna pattern (see Figure \ref{fig:rxfacing}). The UAV moves at the speed of 20m/s, on a cyclical, dumbbell-shaped path. 
Interestingly, results show that receivers experience different packet loss rate due to the UAV movement. More importantly, it indicated that losses are not correlated over the flight path. For example, one of the receiver, receives packets in the northwest quadrant while the other does not. Therefore, utilizing multiple receivers can enhance ground to air communications up to 25\%.
%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%
Authors in \cite{5948706} assumed that the Rician channel model fits best for the ground to air communications at mid or low altitudes, while Loo model \cite{loo681373} can be used at high altitudes. Both Rician and Loo model is improved and extended in this work and then a Markov-process transmission based on altitude and environmental parameters is proposed for ground to air communications. 
The ground to air channel is described using fading type, Doppler effect and the delay in \cite{5267877}. A two ray Rician model is used and improved by using turbo encoding. Simulations in MATLAB represents a vary good BER performance. It also shows that the delay component approximate follows the Rayleigh fading model. 

Experimental and simulation works are summarized in Table \ref{tbl:channel_exp} and \ref{tbl:channel_simul}, respectively.


\subsection{Air-to-Air}
Technically speaking, there are many reasons to investigate the air to air channel modeling. 
%\begin{itemize}
%	\item \
	First of all, due to the low cost and recent development of UAVs, deploying multiple number of them in a network becomes more practicable. In such networks, UAVs need to communicate with each other to achieve the coordination \cite{Bekmezci2013FANETs}.
%	\item \
	 Additionally, it was shown that multi-tier drone structure can improve the system performance significantly comparing to the traditional single-tier drones \cite{ikram2017tier,7744808}. Different types of drones can be used in a multi-tier drone networks, which is comparable to the existing  heterogeneous network composed of macro cells, small cells and femtocells. The nature of multi-tier drone networks requires communication and cooperation between drones at different tiers.
%	 \item \
	 Furthermore, the rapid growth of drones in cellular network created a new type of UE, called drone UE \cite{3gpp_RP_170779}. Besides the traditional ground users, the flying users will need to operate in the air, through an air to air channels.
%\end{itemize}

Here, we mentioned three reasons among others to highlight the importance of air to air channel modeling, however, there are few works in the literature exploring it.
Generally, researchers utilized experiment or simulation in order to find the best channel model. We first review some of the experimental results.

Goddemeier et al. \cite{7414180} proposed an extension of Rician model for the air to air communications. As a result, they conducted experiments with two UAVs to identify the required parameters for the extended model.
%They first evaluated the impact of distance between UAVs, where two UAVs are located at the height of 35m, and their distance varies from 25m to 225m. The experiment results indicate that the measured RSS decreases slowly-following a Free-Space model-when the distance increases. In order to realize the impact of drones' altitude, another experiment is done with two UAVs at a fix distance of 50m. Three different altitudes (10m,20m, and 40m) are considered for this experiment. According to the results, a higher variance in RSS can be observed in low altitudes, due to the strong multipath, where in higher altitudes, the direct LoS is dominated. Moreover results show that  the influence of the altitude and variance decreases exponentially.
They evaluated the impact of drones' altitude where two UAVs located at a fix distance of 50m from each other. Three different altitudes (10m, 20m, and 40m) are considered for this experiment. According to the results, a higher variance in RSS (received Signal Strength) can be observed in low altitudes, due to the strong multipath, where in higher altitudes, the direct LoS is dominated. Moreover results show that  the influence of the altitude and its variance decrease exponentially.
A height dependent formula is then proposed to reflect the influence of scattered path in a Rician model as follows:
\begin{equation}
\sigma=a*h^b+c
\label{eq:a2a_rice_height}
\end{equation} 
where $a,b$ and $c$ are fitting parameters based on experimental results, and $h$ denotes the altitude. $\sigma$ represents the impact of scattered path in the original Rician model. 

Field experiments to estimate the path loss exponent for air to air communication in wireless sensor networks using two hexacopter are done in \cite{7470935}. The path loss exponent is estimated using the measured Received Signal Strength Indicator (RSSI). A path loss exponent of 2.05 is reported for A2A links at the height of 20m, which is very close to the free space path loss model. (Free Space path loss = 2). Additionally, the measured path loss exponent for ground to air, air to ground, and ground to ground links indicate the differences between these links. The measured value for various links is reported in Table \ref{tbl:estimaedpathlossallLinks}.

\begin{table}[]
	\setlength\extrarowheight{5pt}
	%\setlength\arrayrulewidth{1pt}
	\centering
	\caption{Estimated path loss exponent for different links \cite{7470935}}
	\label{tbl:estimaedpathlossallLinks}
	%\rowcolors{1}{gray!25}{white}
	\begin{tabular}{|l|l|l|l|l|}
		\hline
		\textbf{Link} &\textbf{A2A}&\textbf{A2G}&\textbf{G2A}&\textbf{G2G}\\ \hline
		\textbf{Path Loss Exponent} &{2.05}&{2.32}&{2.51}&{3.1}\\ \hline
	\end{tabular}
\end{table}

%\paragraph{Experimental}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
	\centering
	\caption{Experimental studies for channel modeling}
	\label{tbl:channel_exp}
	\begin{tabular}{|m{0.7cm}|m{0.7cm}|m{2.5cm}|m{1.5cm}|m{1.5cm}|m{3cm}|m{3.5cm}|}
		\hline
		\textbf{Type}                 & \textbf{Ref.} & \textbf{Frequency/Protocol} & \textbf{Altitude} & \textbf{Environment} & \textbf{Experiment Details} & \textbf{Objective} \\ \hline
		\multirow{3}{*}{\textbf{A2G}} &     \cite{qualcommuavtr}          & PCS, AWS, and 700MHz     & below 120m    &   mixed suburban (California)  &  Custom designed quadrotor drone (5m/s)               & Enhance the understanding of aerial communications   \\ \cline{2-7} 
		& \cite{7357682}        &   970Mhz (L-band), and 5060MHz (C-band)   &   560m  &   Near-urban (Cleveland) &          S-3B Viking aircraft         &    Characterizing the channel for air to ground communication           \\ \cline{2-7} 
		& \cite{8048502}        &   850Mhz, LTE &    15,30,60,90, and 120 m  &  suburb in
		Victoria, Australia &         one commercial UAV, 4.8m/s, sony Xperia phone for logging        &  Modeling the excessive path loss exponent over the terrestrial model      \\ \cline{2-7} 
		&       \cite{7936620}        &    800MHz, LTE &    15,30,60, and 120 m &  Denmark   &    One commercial UAV , 15km/h            & Modeling the path loss exponent and shadowing           \\ \hline
		%%%%%
		\multirow{3}{*}{\textbf{A2A}} & \cite{7414180} &  2.4GHz, IEEE 802.11   &  Below 50m   &  -   & Two AscTec Firefly Hexacopter UAVs  &   Studying the impact of distance       \\ \cline{2-7} 
		& \cite{7470935}                   &  ZigBee 802.145.4   &  Below 20m   &     -             &      Two Hexacopters   &   Measuring path loss exponent    \\ \hline 
		%%%%%
		\multirow{2}{*}{\textbf{G2A}} &   \cite{5700251}           &  802.11b/g    &   75m  &     &  Fix-wing fuselag                &       Measuring the diversity in G2A links        \\ \cline{2-7} 
		& \cite{7470935}                   &  ZigBee 802.145.4   &  Below 20m   &     -             &      Two Hexacopters   &   Measuring path loss exponent    \\ \hline
	\end{tabular}
\end{table*}

%\paragraph{Simulation}
\begin{table*}[]
	\centering
	\caption{Simulation studies for channel modeling}
	\label{tbl:channel_simul}
	\begin{tabular}{|m{0.7cm}|m{0.7cm}|m{2.5cm}|m{1.5cm}|m{1.5cm}|m{3cm}|m{3.5cm}|}
		\hline
		\textbf{Type}                 & \textbf{Ref.} & \textbf{Frequency} & \textbf{Altitude} & \textbf{Environment} & \textbf{Simulation Details} & \textbf{Description} \\ \hline
		\multirow{3}{*}{\textbf{A2G}} &  \cite{7037248}  &700MHz, 2000 MHz and 5800MHz      & 200m-3000m    &  Suburban, Urban, Dense and Highrise Urban   &  MATLAB, Wireless InSite, One quasi-stationary UAV                &    Finding a generic path loss model based on urban parameters           \\ \cline{2-7} 
		&      \cite{4151547}      &  5GHz    &    100m, 200m, 500m, 1000m and 2000m & Bristol area with irregular street    &      Ray tracing software            &    Modeling LoS probability  based on  building geometry                 \\ \hline
		\multirow{3}{*}{\textbf{A2A}} &    \cite{6167508}          &   --   & --    & --    &   Two UAVs (22m/s) in the simulated area       &       Modeling the packet dropout using Rician channel model        \\ \cline{2-7} 
		&     \cite{5700253}         & 2.4GHz (80MHz BW)      &  --   & --    &        Three UAVs, one as a relay          &   Modeling the bit rate over different channel models            \\  \hline
		\multirow{2}{*}{\textbf{G2A}} & \cite{5267877}&  5GHz    &   --  &  --    &  MATLAB , one aircraft (300m/s)              &  Studying the characters of channel such as
		the Doppler, and the type of fading     \\ \hline
	\end{tabular}
\end{table*}

Besides the experiments, channel specifications can be examined through analytical model and simulations. For example, a combination of two state Markov model and Rician model is proposed in \cite{6167508} to model the packet dropout in air to air communication. Due to the existence of a dominant LoS path for UAV communications, the Rician model is selected for the simulation. The proposed Markov model has two states, a good and a bad one. When the channel is in the good state it follows the Rician model, while in the bad state the probability of packet dropout is 1. The model is then simulated  using two UAVs which are moving with the speed of 80km/h (22m/s).
It is shown that the error probability and the packet dropout increases as the distance between UAVs increases. Moreover, results indicate that the proposed model can simulate the error in UAVs communications perfectly.

Abualhaol et al. \cite{5700253} derived a close form to express the outage probability and the average achievable bit rate over various types of fading channels. In the considered network, multiple UAVs send their data to a relay UAV, and then the relay UAV transmits data to a ground base station. A minimum bit rate is defined for each communication link. Different sub-channels are assigned to UAVs to avoid interference. Rayleigh, Nakagami-m, and Weibull fading channels are considered in this paper, where utilizing the model depends on the operation environment. For example, Rayleigh fading is more appropriate for low altitude crowded area applications, where Nakagami-m and Weibull fading are more acceptable for high altitude and open space environments. The proposed model is then evaluated through simulation with three UAVs, operating in 2.4GHz band and the bandwidth of 80MHz. Results reveal that the simulations is compatible with the analytical model, however, the bit rate approximation has the highest degree of accuracy with Nakagami-m model.

Experimental and simulation works are summarized in Table \ref{tbl:channel_exp} and \ref{tbl:channel_simul}, respectively.


\subsection{Summary}
%According to the above discussion, there are several studies working on channel modelling for aerial communications. However, still many challenges remain unsolved. For example, the interference and Doppler effect is ignored in many articles. Additionally, experimental results are mainly limited to one UAV, while more field experiments utilizing  multiple UAVs with different characteristic is needed.
%In order to have a more accurate channel model the impact of weather, temperature, and wind are also needed to be considered \cite{ikram2017tier}.

According to the above discussion, there are several ongoing research on channel modelling for aerial communications. However, still many challenges remain unsolved. For example, the interference and Doppler effect is ignored in many articles. Additionally, experimental results are mainly limited to one UAV, while more field experiments utilizing  multiple UAVs with different characteristic is needed.
In order to have a more accurate channel model the impact of weather, temperature, and wind are also needed to be considered \cite{ikram2017tier}. Moreover, potential extensions of the 3GPP channel model \cite{3GPP36777} can be proposed and discussed by future works. 

\begin{landscape}
\begin{table*}
\centering
\caption{Summary of the most representative current UAV regulations.}
\label{tbl:regulsummary}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		Country & Applicability & \tabincell{c}{Technical\\Requirements} & \tabincell{c}{Operational\\Limitations} & \tabincell{c}{Administrative\\Procedures} & \tabincell{c}{Human\\Resources} & \tabincell{c}{Ethical\\Constraints}\\
		\hline
		Australia & \tabincell{c}{Classification:\\Weight/Purpose} & N/A & \tabincell{c}{Minimum distance to people: 30m\\Minimum distance to airport: 5.5km\\height limit: 120m} & \tabincell{c}{Insurance\\recommended} & \tabincell{c}{$>$2kg:\\License\\required} & \tabincell{c}{Respect\\privacy}\\
		\hline
		UK & \tabincell{c}{Classification:\\Weight/Purpose} & \tabincell{c}{Collision\\avoidance:\\for special\\operations} & \tabincell{c}{Minimum distance to people: 50m\\Minimum distance to\\congested area: 150m\\Maximum flight height: 122m} & \tabincell{c}{Approvals\\vary for \\different\\operations} & \tabincell{c}{Pilot\\Competency} & \tabincell{c}{Respect\\privacy\\and data}\\
		\hline
		US & \tabincell{c}{Classification:\\Weight/Purpose} & N/A & \tabincell{c}{Minimum distance to airport: 8km\\Maximum flight height: 122m} & \tabincell{c}{$>$25kg:\\Operational\\certificate\\required} & \tabincell{c}{Certificate\\required} & \tabincell{c}{Respect\\privacy\\related\\laws}\\
		\hline
		China & \tabincell{c}{Maximum\\weight: 7kg} & N/A & \tabincell{c}{Minimum distance to\\other aircraft: 10km} & \tabincell{c}{Operational\\certificate\\and registration\\required} & \tabincell{c}{Certificate\\required} & \tabincell{c}{N/A}\\
		\hline
		Chile & \tabincell{c}{Classification:\\Weight} & \tabincell{c}{Many special\\demands} & \tabincell{c}{Minimum distance to people: 30m\\Maximum flight height: 130m} & \tabincell{c}{Flight\\authorization\\required} & \tabincell{c}{License\\required} & \tabincell{c}{N/A}\\
		\hline
		\tabincell{c}{South\\Africa} & \tabincell{c}{Classification:\\Weight/\\Visibility} & \tabincell{c}{N/A} & \tabincell{c}{Minimum distance to people: 50m\\Maximum flight height: 122m} & \tabincell{c}{Operational\\certificate\\and registration\\required} & \tabincell{c}{License\\required} & \tabincell{c}{N/A}\\
		\hline
	\end{tabular}
\end{table*}
\end{landscape}

==> CostModel.tex <==
\graphicspath{{Figures/}}
\section{Paradigm-Shifting Cost Model of Drone-cells}
\label{s:CostModel}

Next generation cellular networks are expected to be 50 times more cost effective than 4G \cite{roh20145g}. Therefore, cost saving has become a major challenge for conventional cellular operators. Costs of conventional cellular operators usually include capital expenditure (CAPEX) and operational expenditure (OPEX). CAPEX comprises acquisition, design and construction of site, purchase and implementation of equipment, etc. OPEX is made up of recurring costs such as site maintenance and rental, personnel expenses, electricity, etc. Fig.~\ref{fig: CAPEX/OPEX} depicts the CAPEX/OPEX breakdown in developed countries.

%	\begin{figure}[htb] 
%	    \centering
%	    \includegraphics[width=1\linewidth]{Figures/CAPEX.png}\\
%	    \includegraphics[width=1\linewidth]{Figures/OPEX.png}
%	    \caption{CAPEX/OPEX breakdown in developed countries \cite{instance1290}}
%	    \label{fig: CAPEX/OPEX} 
%   \end{figure}

\begin{figure}
    \centering
    \subfigure[CAPEX]{
    \begin{minipage}[b]{0.5\textwidth}\includegraphics[width=\linewidth]{CAPEX.png}
    \end{minipage}
    }
    \subfigure[OPEX]{
    \begin{minipage}[b]{0.5\textwidth}\includegraphics[width=\linewidth]{OPEX.png}
    \end{minipage}
    }
 \caption{CAPEX/OPEX breakdown in developed countries \cite{instance1290}} 
 \label{fig: CAPEX/OPEX}
\end{figure}

It can be observed from Fig.~\ref{fig: CAPEX/OPEX} that cellular operators spend more than half (52\%) of their CAPEX on site acquisition and construction, which is followed by the costs of BSs, network testing, power and backhaul. However, CAPEX breakdown for drone-cells is expected to be quite different. With flying drones carrying cellular BSs, site-related costs could be significantly reduced or even completely removed. While the costs of BSs and network testing for drone-cells should increase compared to employment of terrestrial BSs due to the purchase and operation of drones. Overall, drone-mounted BSs have the potential to slash down the CAPEX of cellular operators by significantly reducing the site-related costs, which currently account for the lion's share of the CAPEX.

In terms of OPEX, site-related costs also occupy a major proportion. Site rental makes this percentage even larger, if cellular operators do not own their sites \cite{meddour2011role}. As it can be seen from Fig.~\ref{fig: CAPEX/OPEX}, land rent constitutes up to 42\% of cellular operators' OPEX in developed countries. Authors in \cite{lang2009business} also reveal that site rental dominates the OPEX of cellular operators. Moreover, due to site shortage and stricter environmental regulations, site rental is becoming increasingly expensive \cite{RNSLTE}. Furthermore, promising 5G techniques such as ultra-dense cell deployment make the costs of site rental even higher since a large number of BSs will be required. When using flying BSs, the most expensive part of OPEX could be greatly reduced, at the cost of potentially higher expenses on electricity and backhaul. There will also be some additional costs such as annual registration fee for drones, flying insurance and their battery replacement.

Compared to traditional cells equipped with terrestrial BSs, cost model of drone-cells is paradigm-shifting. With BSs mounted on flying drones, both CAPEX and OPEX of conventional cellular operators could be significantly reduced by saving site-related costs, which contributes to the improvement of cost effectiveness for conventional cellular operators. In addition, when employing terrestrial BSs or relays to extend the cellular coverage, cell reorganization is required and could be expensive. This cost could be saved by deploying flying BSs/relays instead. Moreover, new business models may also emerge. For example, the deployment of drone BSs could follow the time-variant movement of people/cellular UEs, which could be achieved by easy and cheap shipping means such as public transportation systems (e.g. trains and buses). For another example, such paradigm-shifting cost model also enables some new cellular operators to provide opportunistic communication services. For drone fleet owners such as Google and Amazon, goods and data could be delivered simultaneously by flying drones following designated routes.

==> taxonomy.tex <==
\section{Taxonomy for UAVs in Networks} 
\label{sec:chapter2_bkgr_modelandprotocols}

Networks consisting of UAVs have unique features which are separating them from other types of networks. Differences between networks of UAVs and other forms of network such as MANET and VANET are summarized in \cite{7317490}.
%Figure \ref{fig:adhocvsfanet} \cite{7317490}. 
In particular, a new form of MANET with unique characteristics like mobility, channel model, and energy consumption is defined in \cite{Bekmezci2013FANETs} called FANET. Nodes in FANET are UAVs, and UAV-UAV communications exist beside UAV-infrastructure and UAV-ground user communications. Example of FANET is shown in Figure \ref{fig:fanet_my}.

\begin{figure}
	\centering
	\includegraphics[width=0.6\linewidth]{Figures/fanet_my}
	\caption{Example of FANET including UAV-to-UAV and UAV-to-user communications}
	\label{fig:fanet_my}
\end{figure}

%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\linewidth]{Figures/adhoc_vs_fanet}
%	\caption{{\color{red}comparing MANET, VANET and UAV networks \cite{7317490}}}
%	\label{fig:adhocvsfanet}
%\end{figure}
 

The wireless data-link model for UAS  and their challenges are discussed in \cite{6214697}. Two of the main characteristics of UAS that need to be considered in data-link design is long distance and high speed of UAS communication. Assigning L-band (960 - 1164 MHz) for UAS communication is addressed in \cite{6214697}, considering the possible challenges and issues. Using high frequency and large distances increase path loss and need more transmission power to make a successful communication. Moreover, lower frequencies are a better choice for high-speed mobility applications because of smaller Doppler spread. Another important parameter in frequency selection for UAS is the effect of weather. These challenges along with two duplexing methods (TDD and FDD) are reviewed for designing an efficient data-link for the UAS using proposed L-bands. 
%High altitude platform (360Km) and high speed systems (1000km/h) are considered in this work.


%\subsection{Characteristics}
In the following, some of the main taxonomies used in the network of UAVs are described \cite{Bekmezci2013FANETs,6564779}:

\subsection{Channel Model}
Air to ground communication model could be different to the other existing models. Some studies are trying to find a realistic channel model for UAV communications. Filed measurements are conducted in \cite{7936620}, to analyze the effect of UAV height on channel modeling and propagation. Their studies shows that a height dependent model for UAV communication is needed, as the path loss exponent decreases by increasing the UAV height. In this study, the UAV height goes up to 120m.
An investigation into specific path loss and propagation model for UAV communications has been done in \cite{7037248,4483593,6685719}. Additionally, a propagation model using LAP in urban environments is presented in \cite{7037248,6863654}. These studies derived a closed-form expression based on elevation angle to present the probability of having LoS connection for LAP. The expression is according to the ITU model \cite{ITU} and environmental parameters. The elevation angle of a connection between a UAV and users are shown in Figure \ref{fig:elevationangle_my}. A shadowing model for HAP in built-up areas is modeled in \cite{4483593,loke2015internet}. 

\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{Figures/elevationangle_my}
	\caption{Elevation angles for connections between a UAV and users }
	\label{fig:elevationangle_my}
\end{figure}

Moreover, the impact of different weather condition \cite{6685719}, various urban area \cite{loke2015internet} are also studied by researchers.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Power Consumption}
UAVs battery consumption is of paramount importance for UAV network, as it can limit the network lifetime \cite{7317490}. Energy efficient protocols and models are required to be used in UAV systems. Separate from communication energy, the aircraft battery consumption needs to be taken into account in designing protocols and models of UAV networks. More detail on the energy consumptions and proposed alternative are described in Section \ref{subsec:challenge_energy}.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Regulation}
Due to security and privacy issues some regulations and licensing on using UAVs are legislated by FAA \cite{faaregulations,faawikiusa}. For example, according to FAA rules \cite{faaregulations}, small UAVs can not fly higher than 400 feet above the ground level. Moreover, the maximum speed of 100mph is defined for small UAVs.


\subsection{Mobility Model}
While the users' mobility pattern in mobile networks such as MANET and VANET are more restricted and predictable, UAVs have different mobility pattern. They can change their speed, altitude, and heading and create various trajectories. Zarifneshat et al. \cite{Zarifneshat20131078} presented a new realistic mobility model that can be used for entities able to change their speed and direction.
% According to real models, when a user decides to change its direction, deceleration and acceleration are needed.
Based on the presented model by Zarifneshat et al. \cite{Zarifneshat20131078}, a change of direction by a user, can be predicted based on speed variation. The model presented in this paper is applicable for UAVs as well.
%
More importantly, various sources of uncertainties exist in UAVs and their mobility such as time delay, external disturbances, nonlinear dynamic, etc. \cite{Dydek20131043}. An exact controller is needed to force UAVs to follow the recommended path and reduce the distance and tracking error \cite{6220873}. Mobility model for a group of UAVs is becoming even more complicated. Because of the fast development of UAVs, their cost is also reducing, creating the opportunity to use a swarm of UAVs. A method to control the movement of multiple UAVs, reduce the collision, and minimize the deviation from the commanded trajectories is presented in \cite{Dydek20131043}.
%
Additionally, the mobilities of UAVs may cause intermittent link, and network partitioning. As a result, finding an efficient routing protocol becomes an important issue for UAV networks \cite{7317490}. Applicability of the existing routing protocol for UAV networks is discussed in \cite{7317490}.%, summarized in Figure \ref{fig:routingprotocols}.
  
%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\linewidth]{Figures/routingprotocols}
%	\caption{{\color{red}Applicability of existing routing protocol for UAV networks \cite{7317490}} }
%	\label{fig:routingprotocols}
%\end{figure}


%\be
%\item \textbf{High Mobility}:
%UAVs have a higher degree of mobility compared to the existing networks, risen to significant communication challenges such as being unstable and facing temporary disconnection.
%
%\item \textbf{Node Density}: 
%Normally, the number of UAVs in a FANET is less than the number of nodes in other networks.
%
%\item \textbf{Topology Change}:
%Change of topology is more frequent than other networks, a direct result of higher mobility of UAVs.
%\ee





%\azade{read these papers for challenges and opportunities:
%}%\cite{6564779}, \cite{ZengZL16a}}




%There are several advantages of using UAVs including cost-efficiency, availability, agility and Survivability. However, there are still challenges in using UAVs need to be addressed such as national regulations, routing, and path planning. In the following section we review the existing challenges and solutions 

%
%Authors in \cite{7423671} presented a conceptual model for Internet of Drones architecture, developed a vocabulary of concepts for describing the architecture and identified the relevant
%components of it as well as deciding on the boundaries of the architecture.
%
%Another study on internet of drones is conducted in \cite{7465674}. The challenges to have a safe, secure, and reliable large-scale public drone operations, (airspace awareness, non-LOS control, augmentative control, and collision avoidance) is studied well. Also, Geocast Air Operations Framework (GAOF), as an option to address these challenges is introduced.
%
%Outlining the opportunities and challenges involved in deploying UAV networks in the sky for civilian applications is presented in \cite{Namuduri2013}.
%
%When using multiple UAVs that need to communicate, there would be Broadcast Storm Problem (BSP). UAVs may need to communicate together to find out about neighbors' position to avoid collision. In \cite{7427915} some of the methods used in MANET and VANET to handle BSP are considered for FANET as well. Three different typologies are analyzed and the performance of BSP mitigating methods are studied through the number of received messages, the number of saved re-broadcasted messages and the number of redundant messages. 
%
%The wireless DataLink model for Unmanned Aircraft Systems and their challenges is discussed in \cite{6214697}. Two of the main characteristics of Unmanned Aircraft Systems (UAS) that need to be considered in datalink design in long distance and high speed of UAS communication. In this paper, assigning L-band (960 - 1164 MHz) for UAS communication is discussed considering the challenges. Using highe frequency and high distances increases path loss and need more transmission power in order to make a susses communication. Moreover, lower frequencies are better choice for high-speed mobility applications because of smaller Doppler spread. Another important parameter in frequency selection for UAS is the effect of weather. These challenges along with two duplexing method (TDD and FDD) are discussed for designing an efficient datalink for the UAS using proposed L-bands. High altitude platform (360Km) and high speed systems (1000km/h) are considered in this work.
%
%.
%
%\cite{7470932} summarized the outcome of ABSOLUTE project on using aerial LTE Advance base station. It has been shown that using aerial base station is very encouraging during unexpected events. At first different technology to be used as aerial low altitude base station is studied, current technologies include Drones, Aircrafts, Airship and Helikite. Different parameters such as energy consumption, altitude, payload, safety and .. are compared for possible platforms.Moreover, the air to ground channel model is also discussed in this paper where the probability of having a line of sight depends on the elevation angle of aerial base station. There are still some limitation and challenges in aerial network consisting lack of testbeds, power consumption, regulation laws.
%
%Using UAVs in public and civil application is promising, however, there are many issues related to UAVs that must be considered. \cite{7317490} addressed the open problems and the most important challenges in UAVs usage. At first, UAVs networks are compared with MANET and VANET and their difference and common features are distinguished. It is mentioned that although these kind of networks share some features, there are important unique properties for UAVs network.
%Routing in UAV network has more requirement than other networks because of energy constraint and high mobility. Existing routing protocol are discussed to see how they could be efficient for UAV network and what are the necessary changes. 
%energy constrain is also one of the important issues in UAV network. Energy conservative methods applicable in different network layer protocols are discussed in this paper.
%Seamless handover, dynamic topology and intermittent links are additional features of UAV network that need to restudy. Moreover, in this paper, UAV network are categorized based on their application in three group namely Internet delivery, sensing and attack. 
%
%\cite{5624356} investigate the channel model for air to ground communication in urban area. They evaluated  which channels model fits the best considering the height of aerial base stations.





==> uavinnoncellular.tex <==
\subsection{UAVs in Non-Cellular Networks}
 \label{sec:bkrg_uavinnoncellular}
In this section, we review the recent works in non-cellular networks in which UAVs are used. Application of UAVs in WSN, MANET, VANET, and other wireless networks such as WiFi are provided in the following subsection. Then, a summary of articles and their applications are listed in Table \ref{tbl:uavsinnoncellular}. 

\subsubsection{WSN}

%\subsubsection{Data Collection}
Collecting data in a sensor network using UAVs in remote areas and areas with limited access to human is studied in \cite{Yoo2016140}. The sensor network area is divided into three different categories including prohibited area, areas for data collection and area just to fly over them. The flying path is optimized considering energy consumption, flying time, and sensor density. A weighted sum utility function is defined given different weight for the above parameters. A genetic algorithm is used and analyzed through numerical results. UAVs are used to collect data from sensor nodes in an energy efficient mode in \cite{7192644}, \cite{6848000} and \cite{6867394}. A UAV collects data from cluster heads \cite{6848000} while moves in a circular way characterized by altitude, radius, and speed. Each cluster head can communicate with the UAV considering five different modulations (no transmit, PSK, QPSK, 16-QAM, and 64-QAM), switching between modulation mode is according to fixed SNR values. A time slot allocation problem to reasonably maximize the energy efficiency of data collection is modeled in this work. The same problem of \cite{6848000} with multiple UAVs and a game theoretic model is studied in \cite{6867394}. In \cite{7192644}, multiple UAVs which are moving in a circular pattern are collecting data from sensors and forward them to a remote base station. A transmission schedule is evaluated for UAVs to improve the energy efficiency while guarantee packet success rates.

%\begin{figure}
%	\centering
%	\includegraphics[width=0.4\linewidth]{Figures/data_collection.pdf}
%	\caption{Collecting data using cooperative UAV relays in WSN\cite{7192644}}
%	\label{fig:bkgr_datacollection}
%	%\vspace{-0.4cm}
%\end{figure}

Another novel application of UAVs in WSN is proposed in \cite{7350057}. Due to the high cost and error in reading power meters manually, this paper proposed a protocol for meter reading using UAVs. Cognitive radio scheme is used in \cite{7090210}, when UAVs collect data from static sensors. It is shown that using cognitive radio scheme can improve network performance.
%\subsection{Enhancing System Throughput}

UAVs can also be used in broken wireless sensor networks where sensors are placed in inhospitable places to monitor the area. In these networks, a node failure could create a major problem in monitoring and communication with other nodes. Fast deployment of UAVs can help in mitigating the problems cause by node failure, and build more resilient networks to natural disasters. For instance, a UAV can act as a data mule when some sensors of urban river monitoring network fail due to floods or landslides \cite{6979956}. Deployment of UAVs to recover a failure in WSN and create connectivity between isolated components is also studied in \cite{5676621,7502327}.

A network consists of one observation UAV, and one relay UAV is used to maximize the transmission throughput from the observatory area to a fixed base station in \cite{7510735}. The observation UAV moves freely over the observation area, collects information, and transmits it to the base station through a UAV relay. The relay UAV finds an optimal location to stay and changes its position after a particular period. The throughput of the UAV network is formulated according to the environmental parameters such as the distance between the observation UAV and the observation area size. Numerical results show that there is an optimal location for the relay UAV depending on the size of observation area and the distance from the base station.

%A network of UAVs is used to create a connection between disconnected parts of a WSN in \cite{5676621}. Authors proposed a beacon-based mechanism, where the base station sends beacon messages to UAVs and each UAV broadcast the received beacon. As a result, each UAV can keep the path to the BS. UAVs fly randomly, however when they found out that their connection with the last UAV is about to broken (based on RSSI), they try to change direction in order to improve their connection with the last UAV. Simulation are conducted for 8 UAVs over a 10km by 10km area, with 3km communication range, All UAVs have the same altitude of 250m. Results showed that the proposed method can maintain the connectivity of WSN. \cite{6979956} suggests the using UAVs in maintaining the connectivity of WSN, where node failure happens because of natural disaster. Two main category of UAV usage is considered in this work, namely data mule and router. Real experiment has been done for this proposal.

Stamatescu et al. \cite{7090210} addressed the cognitive radio scheme in a surveillance framework using UAV communications. The UAV monitors the surveillance area, collect data from static sensors and transmit data to the ground base station. It is shown that cognitive radio scheme results in improving availability, network performance, and interference mitigation. UAVs are also proposed to mitigate the impact of failed nodes and increase the
reliability of the linear sensor networks (LSN) in \cite{7502327}. UAVs are sent to specific locations in a
faulty LSN to provide communication relays for some parts of the network. Different allocation strategy models for UAVs on an LSN are evaluated and compared in this work.

\subsubsection{MANET}

UAVs can be used for maintaining the connectivity between users. Especially in MANET, when users are moving the network could be partitioned. Therefore, UAVs can change their location in order to provide full connectivity to the network.
Minimizing the number of required UAVs to maintain the connectivity in a MANET is discussed in \cite{6911826}. The problem is formulated by Minimum Steiner Tree model, and then heuristic algorithms are proposed. Given the location of ground users and UAVs, new locations for UAVs is computed taking into account the mobility constraints of UAVs.

Improving the connectivity for mobile ad hoc ground users using one single UAV is addressed in \cite{1683473,4787021}. The UAV is deployed according to the Minimal spanning tree, and its movement is controlled to maintain connectivity. Various type of connectivity including global message, worst case, network bisection, and k-connectivity is studied. Given the location and speed of users, an optimal location for the UAV is calculated, and the UAV moves there. The update rate of the UAV position depends on the mobility degree of the network; however, 10 sec is used for the simulations. It is shown that the proposed algorithm can improve the MANET connectivity remarkably.


UAVs feature agility, autonomous control, and high degree of freedom. Therefore, they can be employed quickly in hard conditions and dangerous places. One of the primary application of UAVs is surveillance coverage along the remote area. Detecting a suspicious moving watercraft is studied as an use-case of UAV surveillance application in \cite{Lilien20143}.


%\begin{figure}
%	\centering
%	\includegraphics[scale=0.4]{Figures/watercraft.jpg}
%	\caption{Detecting a suspicious watercraft using a UAV \cite{Lilien20143}}
%	\label{fig:bkgr_watercraft}
%\end{figure} 

\subsubsection{VANET}
%\subsection{Enhancing System Throughput}
Using UAVs for improving the connectivity and routing in VANET is proposed in \cite{7564747}. Because of the high mobility of vehicles in the roads and large number of obstacles, UAVs can improve the accuracy of connectivity between vehicles. It is assumed that each area of four road segments are covered by one UAV. UAVs can move with the speed of 50-120kmh. %(See Figure \ref{fig:uvar_vanet})

%\begin{figure}
%	\centering
%	\includegraphics[width=0.4\linewidth]{Figures/uvar_vanet.pdf}
%	\caption{An example of a VANET scenario involving UAVs. \cite{7564747}}
%	\label{fig:uvar_vanet}
%\end{figure} 


\subsubsection{Other Wireless Networks}

%%%%%%%%%
One of the main practical application of UAVs is tracking of mobile targets. UAVs can change their altitude, speed, etc. in order to cover targets properly \cite{1661182,DiPugliaPugliese2016,Zorbas201616,ZORBAS201380}. Moreover, UAVs are equipped with cameras that enable them to detect targets and follow them. Pugliese, et al. \cite{DiPugliaPugliese2016} addressed the problem of mobile target tracking using several UAVs where each UAV has a limited energy resource. The objective is to minimize the number of required UAVs to cover all the targets. An optimization problem is formulated to find the location of UAVs to cover targets, and the problem is re-solved whenever the mobility of targets is changed. For simplicity, a set of discrete altitudes and limited possible 2D plane locations are considered for UAVs. Localized and centralized algorithms for this problem is proposed in \cite{Zorbas201616,ZORBAS201380}.

Using UAVs in order to establish emergency communication in the aftermath a disaster is considered as a potential alternative to traditional methods, as well. One possible conceptual architecture is discussed in \cite{6081580}, consisting of a multi-level aerial topology; including a wide range of airborne stations, from quasi-stationary satellites to small UAVs with different mobility patterns. The defined architecture is evaluated by sampling the 2005 Hurricane Katrina disaster use-case; however, the technical challenges and issues are not addressed in this paper. Another system for disaster recovery consisting of three main subsystems (1-end to end communication, 2-formation control, and 3-autonomous navigation) is proposed in \cite{Tuna201427,6421446}. The performance of the system is practically evaluated through real field experiments by one UAV.

Another interesting application of UAVs is monitoring and covering an area of interest \cite{5928811,7101619,Torres2016441}. The target area may include no-flight zones or obstacles. Moreover, other constraints such as flight time, UAV energy consumption, and trajectory could be involved in the applications. Finding a path to cover the area of interest while taking the energy consumption into account, is discussed in \cite{7101619}.
A genetic algorithm solution is proposed by authors to find an optimal trajectory while satisfying the required constraints. Placement of multiple UAVs with directional antennas to maximize the coverage of the given area is the subject of \cite{7486987}, as well. UAVs have the same altitude and transmission power, and the \textit{circle packing theory} is used to formulate the coverage problem. UAVs can be deployed as relays in remote areas to extend the coverage of existing base station for users. By creating multi-hop D2D communications, UAVs cover the area where it is difficult to deploy a land based relay \cite{7122575}.

Collecting data from ground tasks and forwarding the data to a central base station using multiple UAVs in the wireless networks is also analyzed in \cite{5137409}. A game theory model is proposed to form disjoint UAV coalitions for data collection in order to improve the network performance. In this work, a UAV can stop hovering above a task to collect data, and then move toward the next assigned task for data collection. An experimental test when a UAV acts as a relay to transmit information from an underwater vehicle to a ground base station is described in \cite{7063641}. There is a UAV moving in a circular way around an underwater vehicle with the speed of 18m/s. The effect of altitude and flying radius, waves and less ideal conditional like wind and rain are analyzed in this communication.
% Results shows the the main bottleneck in the communication performance is not the UAV altitude, radius and environmental condition.
It is shown that the main feature affecting the communication between underwater vehicle and the UAV is the underwater vehicle capacity.% IEEE802.11g or IEEE802.11b WiFi is used for the communication.

Motion control of multiple UAVs to improve the link capacity between two mobile nodes is studied in \cite{7237535}. UAVs are acting as relay chain between the nodes. They use Artificial Potential Field model to control the speed and heading angle of UAVs. Different heading angle limitation and speed are considered in the simulation. A decentralized motion control for a chain of UAVs to improve the communication between two mobile nodes is also discussed in \cite{6214700}. Each UAV find a location according to the observed communication data (mainly SINR) and move considering the dynamic limitations. An algorithm to decide on the radius and the center of multiple UAVs acting as relays is analyzed in \cite{Takaishi2016} and \cite{7389838}. It is shown that both the distance between UAVs and the UAVs trajectory have a great impact on the communication performance and delay in the network.

%\begin{figure}
%	\centering
%	\includegraphics[width=0.4\linewidth]{Figures/uav_chain}
%	\caption{Communication relay chain system by UAVs\cite{7237535}}
%	\label{fig:uavchain}
%\end{figure}

Moreover, the communication quality between distant nodes can be improved by using UAVs \cite{4225050,chaumette2014proposal}.
%UAV is used as a relay to maximize the throughput between two fixed distant nodes in \cite{4225050}. 
Delay tolerant application is assumed in \cite{4225050}, where a UAV loaded the data from one source node, carried it and then delivered it to the destination while flying in an oval-shaped trajectory. It is shown that using UAV relay generates higher throughput compared with the conventional multi-hop relay communications. Throughput maximization for communication between a fixed source and destination through a mobile relay is studied in \cite{7572068} as well. A relay is mounted on a UAV to act as a mobile relay. Any information received by relay from the source may be buffered until it reached a better location to forward information to the destination; as a result, a longer delay can be expected given mobile relay. The problem is formulated as a non-convex optimization problem to optimize the source/relay power allocation and relay trajectory. Because of nonconvexity of the problem, two sub-problems are considered and solved alliteratively. The first one is to optimize power allocation given a fixed trajectory (Lagrange and KKT), and the other one is trajectory optimization given a fixed power allocation (non-convex, maximizing the lower bound).
%In \cite{7572068}, throughput maximization for communication between a fixed source and destination through a mobile relay is studied. A relay is mounted on a UAV to act as a mobile relay. Any information received by relay from source, may be buffered until it reached a better location to forward information to destination, as a result, longer delay can be expected given mobile relay. The problem is formulated as a non-convex optimization problem to optimize the source/relay power allocation and relay trajectory. Because of non-convexity of the problem, two sub-problem are considered and solve alliteratively. The first one is to optimize power allocation given a fixed trajectory (Lagrange and KKT), and the other one is trajectory optimization given a fixed power allocation (non-convex, maximizing the lower bound). Moreover it is assumed that the start and final point for the relay trajectory is predetermined. The free path loss model is used for communication. Numerical results are presented to evaluate the proposed method. UAV is flying at fixed altitude of 100m with maximum speed of 50m/s. (freq = 5GHz).

An optimal spectrum allocation to maximize the network performance is designed in \cite{7127619,Si2015}, where the network consists of multiple heterogeneous UAVs. UAVs have different computing capabilities, speed, fuel, transmission power, etc. A three layers architecture is considered in these works, including ground users, UAVs, and satellites. Data is collected from ground users and then processed by upper layers. Although UAV-assisted networks are studied in the literature, the main contribution of these works is taking into account heterogeneous UAVs in the network.

Maintaining the connectivity of a mobile node and a fixed base station using a mobile UAV relay is studied in \cite{Ouyang2014313}. This paper addressed the dual-hop communication between the base station and the end user. An algorithm to find the best location for the relay UAV to move there is proposed in this work. The algorithm is frequently run (every 1 second in simulation) to relocate the UAV. Limited turning angle is considered for the UAV in this paper. Results showed that the proposed algorithm can improve the connectivity and dual-hop SNR for a mobile UAV relay.

Furthermore, UAVs can be used for aerial localization. In \cite{6361401}, a waypoint-based route is planned for one UAV in order to fly over the area of interest and locate the mobile targets. A sniffer (Nokia N900) is mounted on the UAV, and the receive signal strength from mobile targets are collected. The flight path is designed to determine the smaller estimated area of the mobile target location. An average 5meters localization accuracy is achievable in this work.

Employing UAVs to establish emergency communication after a disaster event quickly is the subject of several other works such as \cite{7417170}. A mobile relay that could be a UAV received delay tolerant data from the community connected to the internet and forwarded them to other communities by visiting them. The goal is to design a path for the relay and to choose the amount of data that it carries for each community. The problem is formulated as a min-max problem to maximize the minimum performance of each community. The utility function includes the spectral efficiency of each community and an exponential penalty function of delay.

Connecting two separates subnet using a moving UAV relay is addressed in \cite{7562472}, where the UAV flies in a circular trajectory. The feasibility of using the UAV and the performance of both downlink and uplink is evaluated in this work. According to the position of the UAV and its distance from the source subnet, an adaptive communication rate is selected. As a result, their proposed method adaptively optimizes the rate for a given channel model. Results show that significant improvement can be brought by using the variable-rate protocol. Moreover, creating a communication chain for two nodes without line of sight using mobile UAV relays is studied in \cite{Grotli2012}.

Authors in \cite{Kim2008696} investigated on designing a safe path for an autonomous UAV to move to a target position while there is limited information available. The path is the set of way points whose risk is less than a threshold. In this study, the UAV's sensor has a limited range and the location of obstacles and threat change in real-time. It is assumed that the probability of the existence of a threat within a UAV sensor range is known. The proposed algorithm for real time path planning is evaluated through numerical results and various scenarios for one single UAV flying with the speed of 50m/s over 2km of the target area. It is also shown that the proposed algorithm converges to a solution if there exists a path from starting point to the target point. 
Another path planning research for UAVs has been addressed in \cite{Shanmugavel20101084}. This paper has studied the problem of path planning for a group of UAVs starting their trajectory from an initial point, and are desired to reach their destination point simultaneously. The designed path planner has three main phases to generate a feasible path, including satisfying the kinematic constraint, avoiding physical collision and obstacles, and guaranteeing simultaneous arrival.
Moreover, authors in \cite{ZHUONING2010341} studied the path planning problem for a UAV using Fuzzy Virtual Force. The main reason for using virtual force is to plan a path for the UAV with low complexity, applicable for real-time applications. 

Deriving a theoretical model for the propulsion energy consumption of fixed-wing
UAVs as a function of the UAV's flying velocity and acceleration is discussed in \cite{7888557}. It is assumed that the UAV is flying in a circular trajectory. Authors modelled the problem to find the optimal flight radius and speed to improve the energy efficiency of the communication with one ground user. 
An adaptive video streaming is proposed in \cite{Kacianka2015} to be used in UAV networks which suffer from low throughput because of high mobility. In this work, delay is defined as a trigger for using the proposed method, based on Kofler algorithm.

\begin{table*}[]
	\setlength\extrarowheight{5pt}
	%\setlength\arrayrulewidth{1pt}
	\centering
	\caption{Summary of prior UAV works in  non-cellular networks}
	\label{tbl:uavsinnoncellular}
	%\rowcolors{1}{gray!25}{white}
	\begin{tabular}{|m{3.5cm}| m{5.8cm}| m{3.8cm}|}
		\hline
		\textbf{Network} & \textbf{Application} &\textbf{References}
		\\
		\hline
		\multirow{2}{*}{WSN} 
		&Data Collection & \cite{6848000,6867394,7192644,Yoo2016140,7090210,7350057,7510735} \\ \cline{2-3} 
		&Maintaining Connectivity & \cite{6979956,5676621,7502327}
		\\ \hline 
		\multirow{2}{*}{MANET}
		&Maintaining Connectivity& \cite{1683473,4787021,6911826}\\ \cline{2-3}
		&Surveillance & \cite{Lilien20143}
		\\ \hline 
		VANET&Enhancing System Throughput & \cite{7564747}
		\\ \hline 
		\multirow{9}{*}{Others} 
		&Localization & \cite{6361401} \\ \cline{2-3}
		&Enhancing System Throughput & \cite{7237535,6214700,7127619,Si2015}\\ \cline{2-3}
		&Maintaining Connectivity&\cite{Ouyang2014313}\\ \cline{2-3}
		&Target Tracking & \cite{1661182,DiPugliaPugliese2016,ZORBAS201380,Zorbas201616}\\ \cline{2-3}
		&Disaster Recovery & \cite{6081580,Tuna201427,6421446,7417170}\\ \cline{2-3}
		&Coverage and Monitoring & \cite{5928811,7101619,Torres2016441,7486987,7122575} \\ \cline{2-3}
		&Data Collection& \cite{5137409,7063641}\\ \cline{2-3}
		&Maintaining Connectivity&\cite{Grotli2012,7562472}\\ \cline{2-3}
		&Path Planning&\cite{Kim2008696,Shanmugavel20101084,ZHUONING2010341}
		\\ \hline 
	\end{tabular}
\end{table*}
\subsubsection{Research Gaps}

Although there exist few works validating the proposed system through real field experiments \cite{Tuna201427,6421446}, most of them evaluated their proposal using simulation with a small number of UAVs. A variety of parameters such as battery lifetime, the impact of weather and wind, air to ground path loss, etc. have not been studied well in UAV related works. 
Additionally, extending the work into multiple UAV scenarios and overcoming the new challenges can be applied in studies such as \cite{1683473,4787021,4225050,7562472}.
%Moreover, exploring the issues arising with multiple UAVs is one of the fundamental future steps (\cite{4225050,7562472}), especially for the articles including one single UAV.

The mobility pattern of the UAV has a significant impact on the performance and the energy efficiency of UAV networks; however, the impact of UAV degree of freedom such as altitude, speed, and radius are not considered seriously in these papers. 

Moreover, in most of the works, it is assumed that the UAVs are aware of the location of users at any time, and can predict their positions for the next time slot \cite{7237535,1683473,4787021,6911826,7127619}.



